Deep Underground Neutrino Experiment (DUNE), Far Detector Technical Design Report, Volume IV: Far Detector Single-phase Technology

The preponderance of matter over antimatter in the early universe, the dynamics of the supernovae that produced the heavy elements necessary for life, and whether protons eventually decay -- these mysteries at the forefront of particle physics and astrophysics are key to understanding the early evolution of our universe, its current state, and its eventual fate. DUNE is an international world-class experiment dedicated to addressing these questions as it searches for leptonic charge-parity symmetry violation, stands ready to capture supernova neutrino bursts, and seeks to observe nucleon decay as a signature of a grand unified theory underlying the standard model. Central to achieving DUNE's physics program is a far detector that combines the many tens-of-kiloton fiducial mass necessary for rare event searches with sub-centimeter spatial resolution in its ability to image those events, allowing identification of the physics signatures among the numerous backgrounds. In the single-phase liquid argon time-projection chamber (LArTPC) technology, ionization charges drift horizontally in the liquid argon under the influence of an electric field towards a vertical anode, where they are read out with fine granularity. A photon detection system supplements the TPC, directly enhancing physics capabilities for all three DUNE physics drivers and opening up prospects for further physics explorations. The DUNE far detector technical design report (TDR) describes the DUNE physics program and the technical designs of the single- and dual-phase DUNE liquid argon TPC far detector modules. Volume IV presents an overview of the basic operating principles of a single-phase LArTPC, followed by a description of the DUNE implementation. Each of the subsystems is described in detail, connecting the high-level design requirements and decisions to the overriding physics goals of DUNE.

==> generated/req-just-SP-CALIB.tex <==
% This file is generated, any edits may be lost.
\begin{footnotesize}
%\begin{longtable}{p{0.14\textwidth}p{0.13\textwidth}p{0.18\textwidth}p{0.22\textwidth}p{0.20\textwidth}}
\begin{longtable}{P{0.12\textwidth}P{0.18\textwidth}P{0.17\textwidth}P{0.25\textwidth}P{0.16\textwidth}}
\caption{Specifications for SP-CALIB \fixmehl{ref \texttt{tab:spec:SP-CALIB}}} \\
  \rowcolor{dunesky}
       Label & Description  & Specification \newline (Goal) & Rationale & Validation \\  \colhline

\input{generated/req-SP-CALIB-01.tex} % 1
\input{generated/req-SP-CALIB-02.tex} % 2
\input{generated/req-SP-CALIB-03.tex} % 3
\input{generated/req-SP-CALIB-04.tex} % 4
\input{generated/req-SP-CALIB-05.tex} % 5
\input{generated/req-SP-CALIB-06.tex} % 6
\input{generated/req-SP-CALIB-07.tex} % 7


\label{tab:specs:just:SP-CALIB}
\end{longtable}
\end{footnotesize}

==> generated/req-just-SP-INST.tex <==
% This file is generated, any edits may be lost.
\begin{footnotesize}
%\begin{longtable}{p{0.14\textwidth}p{0.13\textwidth}p{0.18\textwidth}p{0.22\textwidth}p{0.20\textwidth}}
\begin{longtable}{P{0.12\textwidth}P{0.18\textwidth}P{0.17\textwidth}P{0.25\textwidth}P{0.16\textwidth}}
\caption{Specifications for SP-INST \fixmehl{ref \texttt{tab:spec:SP-INST}}} \\
  \rowcolor{dunesky}
       Label & Description  & Specification \newline (Goal) & Rationale & Validation \\  \colhline

\input{generated/req-SP-INST-01.tex} % 1
\input{generated/req-SP-INST-02.tex} % 2
\input{generated/req-SP-INST-03.tex} % 3
\input{generated/req-SP-INST-04.tex} % 4
\input{generated/req-SP-INST-05.tex} % 5
\input{generated/req-SP-INST-06.tex} % 6


\label{tab:specs:just:SP-INST}
\end{longtable}
\end{footnotesize}

==> generated/reqdefs-DP-CALIB.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-CALIB


\def\dpdatavolumelaser{$>\,\SI{37}{TB/yr/10 kt}$}
\def\dpdatavolumepns{$>\,\SI{170}{TB/yr/10 kt}$}
\def\dpefieldcalibcoverage{$>\,\SI{93}{\%}$}
\def\dpefieldcalibgranularity{\SI{10 x 10 x 10}{\centi\metre}}
\def\dpefieldcalibprecision{\SI{1}{\%}}
\def\dplaserpositionprecision{\SI{0.5}{\milli\radian}}
\def\dpneutronsourcecoverage{$>\,\SI{75}{\%}$}


==> generated/reqdefs-DP-CISC.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-CISC


\def\dpcameracoldcoverage{$>\,$80\% of HV surfaces}
\def\dpeleclifetimeprec{$<\,$2.3\%}
\def\dpeleclifetimerange{\SIrange{0.04}{10}{ms} in cryostat, \SIrange{0.04}{30}{ms} inline}
\def\dpinstefield{$<\,\SI{30}{kV/cm}$}
\def\dpinstnoise{$<<\,\SI{1000}\,e^- $}
\def\dpslowcontrolalarmrate{$<\,$150/day}
\def\dpslowcontrolarchiverate{\SI{0.02}{Hz}}
\def\dpslowcontrolnumvars{$>\,\num{150000}$}
\def\dptemprepro{$<\,\SI{5}{mK}$}
\def\dptempstability{$<\,\SI{2}{mK}$ at all places and times}


==> generated/reqdefs-DP-CRP.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-CRP


\def\dpcrpvertprecision{$<\,\SI{1}{\milli\meter}$}


==> generated/reqdefs-DP-DAQ.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-DAQ


\def\dpdaqdeadtime{}
\def\dpDAQreadout{\SI{65}{GB/s} per dual phase detector module}
\def\dpDAQreadoutwindow{\SI{10}{\micro\second} < readout window < \SI{100}{s}}
\def\dpDAQthroughput{\SI{2}{GB/s} average storage throughput; \SI{100}{GB/s} peak temporary storage throughput per dual phase detector module}
\def\dpdatarecord{}
\def\dpdataverification{}
\def\dptriggercalibration{}
\def\dptriggerhighenergy{$>\,$\SI{100}{\MeV}}
\def\dptriggerlowenergy{$>\,$\SI{10}{\MeV}}


==> generated/reqdefs-DP-ELEC.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-ELEC




==> generated/reqdefs-DP-FD.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-FD


\def\dp{}
\def\dpdenonfenoise{$<<\,\SI{1000}\,e^- $}
\def\dpdpadcnumberofbits{\num{12} bits}
\def\dpdpadcsamplingfreq{$\sim\,\SI{2.5}{\mega\hertz}$}
\def\dpdpcathoderesistivity{$>\,\SI{1}{\mega\ohm/square}$}
\def\dpdpcepowerconsumption{$<\,\SI{50}{ mW/channel} $}
\def\dpdpcrpeffgain{\num{6}}
\def\dpdpcrpgaps{$<\,\SI{30}{mm}$ between adjacent CRPs}
\def\dpdpcrpplanarity{$\pm\,\SI{0.5}{mm}$}
\def\dpdpcrpstripspacing{$<\,\SI{4.7}{mm}$}
\def\dpdpcryomonitordevices{}
\def\dpdpdataratetotape{$<\,\SI{30}{PB/year}$}
\def\dpdpdeadchannels{$<\,\SI{1}{\%}$}
\def\dpdpdetmoduptime{$>\,$90\%}
\def\dpdpdetuptime{$>\,$98\%}
\def\dpdpfepeaktime{\SI{1}{\micro\second}}
\def\dpdphvpsripple{$<\,\SI{100}e^-$}
\def\dpdphvsfielduniformity{$<\,\SI{1}{\%}$ throughout volume}
\def\dpdplarimpuritycontrib{$<<\,\SI{30}{ppt} $}
\def\dpdplarncontamination{$<\,\SI{3}{ppm}$}
\def\dpdplarpurity{$>$\,\SI{5}{ms}}
\def\dpdplightyield{$>\,\SI{1}{PE/MeV}$ (at anode), $>\,\SI{5}{PE/MeV}$ (avg  over active volume)}
\def\dpdplocalefields{$<\,\SI{30}{kV/cm}$}
\def\dpdpmindriftfield{$>$\,\SI{250}{ V/cm}}
\def\dpdpmisalignmentfielduniformity{$<\,1\,$\% throughout volume}
\def\dpdpradiopurity{less than that from $^{39}$Ar}
\def\dpdpsignalsaturation{\num{7500000} electrons}
\def\dpdpsntrigger{$>\,\SI{95}{\%}$ efficiency for a SNB producing at least 60 interactions with a neutrino energy >10 MeV in 12 kt of active detector mass during the first 10 seconds of the burst.}
\def\dpdpsystemnoise{$<\,\SI{1000}\,e^-$}
\def\dpdptimeresolutionpds{$<\,\SI{1}{\micro\second}$}


==> generated/reqdefs-DP-HV.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-HV


\def\dphvdbredundancy{$>\,\num{2}$ HVDB chain}


==> generated/reqdefs-DP-INST.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-INST


\def\dpcleanroomspecs{>ISO-8}
\def\dpcoldboxcryo{Independent operation of the four cold boxes}
\def\dphandlingspecs{Fulfill material handling specification}
\def\dpmaterialbuffer{>1 month}
\def\dpundergroundstorage{>4~\dshorts{crp}}


==> generated/reqdefs-DP-PDS.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-PDS


\def\dphitrelativetiming{$<\,\SI{100}{ns RMS}$}
\def\dphitsnr{$>\,\num{5}$}
\def\dppdsanalogrange{$>\,\SI{100}{PE/(ch\times 6\nano\second)}$}
\def\dppmtdarkrate{$<\,\SI{100}{kHz}$}


==> generated/reqdefs-SP-APA.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-APA


\def\spapaactivearea{Maximize total active area.}
\def\spapabadchannels{$<$1\%, with a goal of $<$0.5\%}
\def\spapabiasvoltage{The setup, including boards, must hold 150\% of max operating voltage.}
\def\spapaframeplanarity{$<$\SI{5}{mm}}
\def\spapaunitsize{\SI{6.0}{m} tall $\times$ \SI{2.3}{m} wide}
\def\spapawiretension{\SI{6}{N} $\pm$ \SI{1}{N}}


==> generated/reqdefs-SP-CALIB.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-CALIB


\def\spdatavolumelaser{$>\SI{184}{TB/yr/10 kt}$}
\def\spdatavolumepns{$>\SI{144}{TB/yr/10 kt}$}
\def\spefieldcalibcoverage{$>\SI{75}{\%}$}
\def\spefieldcalibgranularity{$~30\times 30\times 30~$\SI{}{\centi\metre\cubed}}
\def\spefieldcalibprecision{$\SI{1}{\%}$}
\def\splaserlocationprecision{$~\SI{0.5}{\milli\radian}$}
\def\spneutronsourcecoverage{$>\SI{75}{\%}$}


==> generated/reqdefs-SP-CISC.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-CISC


\def\spcameracoldcoverage{$>\,$80\% of HV surfaces}
\def\speleclifetimeprec{$<\,$1.4\%}
\def\speleclifetimerange{\SIrange{0.04}{10}{ms} in cryostat, \SIrange{0.04}{30}{ms} inline}
\def\spinstefield{$<\,\SI{30}{kV/cm}$}
\def\spinstnoise{$<<\,\SI{1000}\,e^- $}
\def\spslowcontrolalarmrate{$<\,$150/day}
\def\spslowcontrolarchiverate{\SI{0.02}{Hz}}
\def\spslowcontrolnumvars{$>\,\num{150000}$}
\def\sptemprepro{$<\,\SI{5}{mK}$}
\def\sptempstability{$<\,\SI{2}{mK}$ at all places and times}


==> generated/reqdefs-SP-DAQ.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-DAQ


\def\spdaqdeadtime{}
\def\spDAQreadout{1.5 TB/s per single phase detector module}
\def\spDAQreadoutwindow{10 $\mu$s < readout window < 100 s}
\def\spDAQthroughput{10 Gb/s average storage throughput; 100 Gb/s peak temporary storage throughput per single phase detector module}
\def\spdatarecord{}
\def\spdataverification{}
\def\sptriggercalibration{}
\def\sptriggerhighenergy{$>$\SI{100}{\MeV}}
\def\sptriggerlowenergy{$>$\SI{10}{\MeV}}


==> generated/reqdefs-SP-ELEC.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-ELEC


\def\spcoldcablesxsec{\SI{6.35}{cm} (2.5")}
\def\spFEMBdatalink{\num{4} at \SI{1.28}{Gbps}}
\def\spgainFEamplifier{$\sim\SI{20}{mV/fC}$}
\def\spnumchannelsFEMB{\num{128}}
\def\spnumFEbaselines{\num{2}}
\def\spnumberFEMBperWIB{\num{4}}
\def\spsyncronizationCE{\SI{50}{ns}}
\def\spWIBdatalink{\SI{10}{Gbps}}


==> generated/reqdefs-SP-FD.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-FD


\def\sp{}
\def\spadcnumberofbits{\num{12} bits}
\def\spadcsamplingfreq{$\sim\,\SI{2}{\mega\hertz}$}
\def\spapagaps{$<\,\SI{15}{mm}$ between APAs on same support beam; $<\,\SI{30}{mm}$ between APAs on different support beams}
\def\spapawireangles{\SI{0}{\degree} for collection wires, $\pm\,$\SI{35.7}{\degree} for induction wires}
\def\spapawirepostolerance{$\pm\,\SI{0.5}{mm}$}
\def\spapawirespacing{\SI{4.669}{mm} for U,V; \SI{4.790}{mm} for X,G}
\def\spcathoderesistivity{$>\,\SI{1}{\mega\ohm/square}$}
\def\spcepowerconsumption{$<\,\SI{50}{ mW/channel} $}
\def\spcryomonitordevices{}
\def\spdataratetotape{$<\,\SI{30}{PB/year}$}
\def\spdeadchannels{$<\,\SI{1}{\%}$}
\def\spdpdetmoduptime{$>\,$90\%}
\def\spdpdetuptime{$>\,$98\%}
\def\spfepeaktime{\SI{1}{\micro\second}}
\def\sphvpsripple{$<\,\SI{100}e^-$}
\def\sphvsfielduniformity{$<\,\SI{1}{\%}$ throughout volume}
\def\splarimpuritycontrib{$<<\,\SI{30}{ppt} $}
\def\splarncontamination{$<\,\SI{25}{ppm}$}
\def\splarpurity{$<$\,\SI{100}{ppt}}
\def\splightyield{$>\,\SI{20}{PE/MeV}$ (avg), $>\,\SI{0.5}{PE/MeV}$ (min)}
\def\splocalefields{$<\,\SI{30}{kV/cm}$}
\def\spmindriftfield{$>$\,\SI{250}{ V/cm}}
\def\spmisalignmentfielduniformity{$<\,1\,$\% throughout volume}
\def\spnonfenoise{$<<\,\SI{1000}\,e^- $}
\def\spradiopurity{less than that from $^{39}$Ar}
\def\spsntrigger{$>\,\SI{95}{\%}$ efficiency for a SNB producing at least 60 interactions with a neutrino energy >10 MeV in 12 kt of active detector mass during the first 10 seconds of the burst.}
\def\spspsignalsaturation{\num{500000} $e^-$}
\def\spsystemnoise{$<\,\SI{1000}\,e^-$}
\def\sptimeresolutionpds{$<\,\SI{1}{\micro\second}$}


==> generated/reqdefs-SP-HV.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-HV


\def\sphvconnectionredundancy{Two-fold}
\def\sppowersupplystability{$>\,\SI{95}{\%}$ uptime}


==> generated/reqdefs-SP-INST.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-INST


\def\spapastoragesd{700 m$^2$}
\def\spcleanroomspecification{ISO 8}
\def\spcleanroomuvfilters{filter $<\SI{400}{nm}$ for $>$ 2 wk exp; $<\SI{520}{nm}$ all else}
\def\splogisticsmaterialhandling{SURF Material Handling Specification}
\def\splogisticsmaterialsbuffer{$>1$ month}
\def\splogisticsshippingcoord{2 wk notice to CMGC}


==> generated/reqdefs-SP-PDS.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-PDS


\def\spapainstall{$>\,\SI{1}{\milli\meter}$}
\def\spenvhumiditylimit{$<\,\SI{50}{\%}$ RH at \SI{70}{\degree F}}
\def\spenvlightexposure{No exposure to sunlight. All other unfiltered sources: $<\,\num{30}$ minutes integrated across all exposures}
\def\splighttightness{Cryostat light leaks responsible for $<\,\SI{10}{\%}$  of data transferred from PDS to DAQ}
\def\spmechcompatibility{$>\,\SI{1}{\milli\meter}$}
\def\spmechdeflection{$<\,\SI{5}{\milli\meter}$}
\def\sppdscable{$<\,\SI{6}{\milli\meter}$}
\def\sppdscablemate{\SI{0}{\milli\meter} separation mechanically allowed}
\def\sppdscleanroomassbly{Class \num{100000} clean assembly area}
\def\sppdsclearance{$>\,\SI{0.5}{\milli\meter}$}
\def\sppdsdarkrate{$<\,\SI{1}{kHz}$}
\def\sppdsdatarate{$<\,\SI{8}{Gbps}$}
\def\sppdsdynamicrange{$<\,\SI{20}{\%}$}
\def\sppdssignaltonoise{$>\,\num{4}$}
\def\spspatiallocalization{$<\,\SI{2.5}{\meter}$}


==> generated/reqdefs.tex <==
% generated file, do not edit\input{generated/reqdefs-SP-FD}
\input{generated/reqdefs-DP-FD}
\input{generated/reqdefs-SP-APA}
\input{generated/reqdefs-DP-CRP}
\input{generated/reqdefs-SP-HV}
\input{generated/reqdefs-DP-HV}
\input{generated/reqdefs-SP-PDS}
\input{generated/reqdefs-DP-PDS}
\input{generated/reqdefs-SP-DAQ}
\input{generated/reqdefs-DP-DAQ}
\input{generated/reqdefs-SP-CISC}
\input{generated/reqdefs-DP-CISC}
\input{generated/reqdefs-SP-ELEC}
\input{generated/reqdefs-DP-ELEC}
\input{generated/reqdefs-SP-CALIB}
\input{generated/reqdefs-DP-CALIB}
\input{generated/reqdefs-SP-INST}
\input{generated/reqdefs-DP-INST}


==> vol-sp/ch-sp-calib/cost.tex <==



\fixme{cost and labor hour tables will be automated in early April, template to come! Anne}

\begin{dunetable}
[Calibration System Cost Summary]
{p{0.15\textwidth}p{0.1\textwidth}p{0.15\textwidth}p{0.4\textwidth}}
{tab:calib-cost}
{Cost Estimates for Different Calibration Subsystems.}   
System & Quantity & Cost (under development) (k\$ US) & Description \\ \toprowrule
laser & 17 & - & high intensity laser source for laser system  \\ \colhline
laser optics module & 20 & -&  insulator ingress into detector and flange interface, mirrors, power, cables for laser system, and positioning system \\ \colhline
Photoelectron system & 4000 & - & includes targets to be mounted, both dots and strips, along with optical fibers to illuminate the photoelectric targets on two cathode planes, on both sides of each  cathode plane \\ \colhline 
DD generator device for \dword{pns}  & 2 &- & neutron source for \dword{pns} system. \\ \colhline
Other \dword{pns} components  & 2 & - & includes moderator, surrounding shielding and neutron monitor \\
\end{dunetable}

\begin{dunetable}
[Calibration labor]
{p{0.25\textwidth}p{0.15\textwidth}p{0.1\textwidth}p{0.08\textwidth}p{0.08\textwidth}p{0.1\textwidth}p{0.08\textwidth}}
{tab:calib-labor}
{Labor Hour Estimates.}
System  & Faculty/Scientist & Post-doc & Student & Engineer & Technician  &  \textbf{Total}\\ \toprowrule
& (hours) & (hours)& (hours)& (hours)& (hours)& (hours)\\ \toprowrule
Ionization Laser system & -& -& -& -& - & - \\ \colhline
Photoelectron Laser system & -& -& -& -& - & - \\ \colhline
Laser positioning system & -& -& -& -& - & - \\ \colhline
\dlong{pns} system & -& -& -& -& - & - \\ \colhline
Physics \& Simulation & -& -& -& -& - & - \\ 
\end{dunetable}

%\todo{SG: need quantity for photoelectron laser in the table 1.6.} KM: Quantity added from Jelena.
Table \ref{tab:calib-cost} shows the current cost estimates for the calibration subsystems. It also shows the quantity associated with each subsystem and a brief description of what is included in the cost estimate. The cost estimates include only materials and supplies (M\&S) and packing and shipping, but not labor and travel costs. One \dword{sp} detector module requires \num{20} ports for the laser (see Figure~\ref{fig:calib-FTmap}); \num{14} ports will each need one laser and one feedthrough interface, but for the \num{6} ports central to the cryostat, one laser will service two ports. According to simulation studies, an \dword{sp} module requires two pulsed neutron systems.

Labor costs depend on personnel category (e.g., faculty, student, technician, post-doc, engineer) and vary by region and institution, so costs are quantified using labor hours needed to complete a given task. Table~\ref{tab:calib-labor} provides estimates of labor hours for each subsystem. 

